Scenic4RL: Programmatic Modeling and Generation of Reinforcement Learning Environments

The capability of a reinforcement learning (RL) agent heavily depends on the diversity of the learning scenarios generated by the environment. Generation of diverse realistic scenarios is challenging for real-time strategy (RTS) environments. The RTS environments are characterized by intelligent entities/non-RL agents cooperating and competing with the RL agents with large state and action spaces over a long period of time, resulting in an infinite space of feasible, but not necessarily realistic, scenarios involving complex interaction among different RL and non-RL agents. Yet, most of the existing simulators rely on randomly generating the environments based on predefined settings/layouts and offer limited flexibility and control over the environment dynamics for researchers to generate diverse, realistic scenarios as per their demand. To address this issue, for the first time, we formally introduce the benefits of adopting an existing formal scenario specification language, SCENIC, to assist researchers to model and generate diverse scenarios in an RTS environment in a flexible, systematic, and programmatic manner. To showcase the benefits, we interfaced SCENIC to an existing RTS environment Google Research Football(GRF) simulator and introduced a benchmark consisting of 32 realistic scenarios, encoded in SCENIC, to train RL agents and testing their generalization capabilities. We also show how researchers/RL practitioners can incorporate their domain knowledge to expedite the training process by intuitively modeling stochastic programmatic policies with SCENIC.

==> macros.tex <==
%\newcommand{\comment}[1]{} 
\newcommand{\sj}[1]{\textcolor{red}{\textbf{{\tiny{SJ!}}}}}

%\newcommand{\scenic}{{\sc Scenic}\xspace}
\newcommand{\scenic}{{\sc Scenic}\xspace}
\newcommand{\scfrl}{{\sc Scenic4RL}\xspace}

\newcommand{\featurespace}{\ensuremath{\textrm{FeatureSpace}}}

\newcommand{\semantics}[1]{\llbracket #1 \rrbracket}
% Space saving List environment for enumerations.
\newcounter{myctr}
\newenvironment{mylist}{\begin{list}{\arabic{myctr}.}
{\usecounter{myctr}
\setlength{\topsep}{1mm}\setlength{\itemsep}{0.25mm}
\setlength{\parsep}{0.1mm}
\setlength{\itemindent}{0mm}\setlength{\partopsep}{0mm}
%\setlength{\itemindent}{0mm}\setlength{\partopsep}{0mm}
\setlength{\labelwidth}{15mm}
\setlength{\leftmargin}{4mm}}}{\end{list}}

% Space saving List environment for itemizing
\newenvironment{myitemize}{\begin{list}{$\bullet$}
{\setlength{\topsep}{1mm}\setlength{\itemsep}{0.25mm}
\setlength{\parsep}{0.1mm}
\setlength{\itemindent}{0mm}\setlength{\partopsep}{0mm}
\setlength{\labelwidth}{15mm}
\setlength{\leftmargin}{4mm}}}{\end{list}}



\newcommand{\supp}{supp}

==> sections/dataset.tex <==

\section{Constructing Dataset with the \scfrl\ Platform}

Our dataset comprises of three categories of data: (1) \scenic{} libraries, (2) \scenic{} programs, and (3) demonstration data generated from semi-expert stochastic \scenic{} Policies.

\subsection{\scenic{} Libraries}\label{scenic_libraries}
As discussed in Sec.~\ref{sec:scenic_background}, \scenic{} libraries consist of three types: model, action, and behavior libraries. The \scenic{} libraries significantly reduces users' time to model complex scenarios by helping them re-use the set of models, actions, and behaviors in the libraries, rather than having to write scenario from scratch. 

% \subsubsection{Model Library}
The \textit{model} library defines the state space. It defines players with distribution over their initial state according to their roles and GRF's AI bot is assigned by default to all player behavior. These prior distribution over the initial state and behavior can be overwritten in the \scenic{} program. The model library also defines region objects such as goal and penalty box regions as well as directional objects in compass directions. The \textit{action} library defines the action space as determined by the GRF simulator. These action space consists of movement actions in eight compass directions, long/short/high pass, shoot, slide, dribble, and sprint. 

The \textit{behavior} library consists of behaviors and helper functions that represent widely used basic skills in soccer. These behaviors include give-and-go, evasive zigzag dribble to avoid an opponent's  ball interception, dribbling to a designated point and shooting, shooting towards the left or right corner of the goal, etc. Additionally, the behavior library also include useful helper functions such as identifying nearest opponent or teammate, whether there is an opponent near the running direction of a dribbler, etc. Please refer to our open-sourced repository for more details.


%\azad{Maybe two snapshots of scenarios that I used in evaluation should also be added here}


\begin{figure*}[!htbp]
    \centering
    \begin{subfigure}[t]{0.23\textwidth}
        \centering
        \includegraphics[height=1.5in, width=1.1in]{sections/figs/new-scenario-1vs1.png}
        \caption{1 vs 1 evasive zig-zag towards the goal and shoot}
        \label{fig:defense_1vs1}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.23\textwidth}
        \centering
        \includegraphics[height=1.5in, width=1.1in]{sections/figs/new-scenario-2vs2.png}
        \caption{2 vs 2 advance the ball towards goal via high pass and shoot}
        \label{fig:defense_2vs2}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.23\textwidth}
        \centering
        \includegraphics[height=1.5in, width=1.1in]{sections/figs/new-scenario-3vs3.png}
        \caption{3 vs 3 left mid-fielder crosses to either player in the penalty box}
        \label{fig:defense_3vs3}
    \end{subfigure}
    ~
    \begin{subfigure}[t]{0.23\textwidth}
        \centering
        \includegraphics[height=1.5in, width=1.1in]{sections/figs/test_pass_and_shoot.png}
        \caption{generalization test scenario for pass and shoot scenario in Fig.~\ref{fig:pass_and_shoot_birdeye}}
        \label{fig:test_pass_and_shoot}
    \end{subfigure}
    \caption{Examples of our new defense scenarios with specific assigned behaviors (left three images) and a test scenario to assess generalization (rightmost). The RL team is yellow and the opponent, blue. The assigned opponent behaviors are highlighted with light blue arrows. Uniformly random distribution is assigned over a specific region for each player. These regions are highlighted boxes.}
    \label{fig:new_scenarios}
\end{figure*}


\begin{comment}
\subsection{\scenic{} programs}
Please refer to our Supplement for detailed descriptions of all our scenarios and policies.

{\bf New Benchmark Scenarios}\label{sec:new_benchmark_scenarios}
We modelled 13 new benchmark scenarios. Nine of them are defense scenarios which are nice complement to GRF's offense-only scenarios. The remaining four scenarios are additional distinct offense scenarios that enriches GRF's benchmark scenarios. We varied the initial state distribution and assigned GRF's AI bot behavior by default. However, if the AI bot did not exhibit the behaviors we expected, we modelled the behaviors of environment agents to create such scenarios. For example, a few of our defense scenarios with specified behaviors are visualized in Fig.~\ref{fig:new_scenarios}. In these scenarios, the opponent AI bot did not exhibit expected behaviors so we specified behaviors in the \scenic{} programs as described in the sub-captions. In 1vs1 scenario, the opponent AI bot was not aggressive enough to attack the goal and was easily pushed out of the penalty box. In 2vs2 scenario, the opponent initially with the ball did not quickly advance the ball to its teammate closer to the goal post via high pass. In 3vs3, the opponent player with the ball on the leftmost side of the field did not cross the ball to its teammates.

{\bf Scenarios for Testing Generalization}  \label{sec:test_ds}
We provide scripts to test generalization of GRF's 5 academy scenarios and all of our 13 new benchmark scenarios from our dataset. The scripts test how robust the trained agents are to perturbations in the initial state. We assigned distribution over the initial state while keeping the formation of players and their behaviors in each scenario intact. For example, for testing generalizability of an RL agent trained in the Pass and Shoot scenario (Fig.~\ref{fig:pass_and_shoot_birdeye}), we instantiated the yellow and the blue players on the symmetric right side of the field instead of the left and kept the other initial state distribution the same (Fig.~\ref{fig:test_pass_and_shoot}). 
%For example, in the 3vs3 defense scenario (Fig.~\ref{fig:new_scenarios}), we instantiated the crossing player on the right side of the field instead of the left and kept the other initial state distribution the same. 

{\bf Probabilistic Scenic Policies and Offline Dataset}\label{dataset:behavior_cloning}
\scfrl\ also allows users to incorporate their domain knowledge by writing probabilistic policies, which can be used as a means to generate rich demonstration data. Users can benefit from using our \textit{behavior} library to write their policies, instead of having to write them from scratch. In our work, we present simple \scenic{}\ policies for three GRF academy scenarios~\cite{kurach2020google} and two of our new benchmark scenarios in which a proximal policy optimization (PPO) algorithm\cite{ppo} had relatively poor training performance. These policies are not to be considered "expert", as they do not solve the scenarios consistently. However, these simple policies can be considered as guidance/ semi-expert policies, which can be utilized for better training. We then generate very small datasets of demonstration from these policies, each containing ~10K samples collected from the successful (i.e. the agent scores) trajectories. Each sample is a $<o,a>$ pair, i.e., specifying the action $a$ the \scenic{} policy took on the observation $o$. In our experiments we show that, such small offline dataset can expedite the RL training significantly.   


\subsection{Towards Crowd Sourced Dataset}
A current limitation of our benchmark dataset is that it does not provide a comprehensive set of scenarios and policies that cover all realistic soccer scenarios and policies on the field. In fact, there are infinitely many different possible scenarios. We address this issue by open-sourcing our platform and dataset, \href{https://github.com/scenic4RL/scenic4rl/tree/v1}{https://github.com/scenic4RL/scenic4rl/tree/v1}, to allow other researchers to contribute their own scenarios and policies as \scenic{} programs. A good crowdsourced dataset will cover much more scenarios than a research group can generate. In fact, the effort to crowdsource a dataset in RL domain has been low due to the lack of support for environment modeling. We share our platform to encourage it. 

\end{comment}

